FREB-TQA: A Fine-Grained Robustness Evaluation Benchmark for Table Question Answering

Table Question Answering (TQA) aims at composing an answer to a question based on tabular data. While prior research has shown that TQA models lack robustness, understanding the underlying cause and nature of this issue remains predominantly unclear, posing a significant obstacle to the development of robust TQA systems. In this paper, we formalize three major desiderata for a fine-grained evaluation of robustness of TQA systems. They should (i) answer questions regardless of alterations in table structure, (ii) base their responses on the content of relevant cells rather than on biases, and (iii) demonstrate robust numerical reasoning capabilities. To investigate these aspects, we create and publish a novel TQA evaluation benchmark in English. Our extensive experimental analysis reveals that none of the examined state-of-the-art TQA systems consistently excels in these three aspects. Our benchmark is a crucial instrument for monitoring the behavior of TQA systems and paves the way for the development of robust TQA systems. We release our benchmark publicly.

==> latex/6-enhance-performance.tex <==
\section{Enhancing robustness of LLM} [Not finished!]
\begin{table}[!h]
\centering
\resizebox{1\columnwidth}{!}{%
  \begin{tabular}{lcccccc}
    \toprule
      & {Emd} & {VP} & {Emd} & {VP} & {Emd} & {VP} \\
    \midrule
    No perturbation &77.71  & 0 &  & \\
    \midrule
    General random &-0.57\pm1.20 & 11.31\pm1.42&-0.46\pm1.96 &12.57\pm2.20 & \\
    Target random& -0.91\pm1.18  & 10.06\pm1.79 &-0.80\pm1.06 &10.40\pm0.84  \\
    Target front &-0.69\pm1.71  & 12.80\pm1.83 & 0.11(1.22)&9.94(1.18) \\
    Target middle & -1.49\pm0.78 & 11.09\pm1.78& -1.14(0.81) &  10.51(0.28) \\
    Target bottom & -0.46\pm1.37 &10.51\pm0.86  &  -1.14(0.89)&   10.14(1.17)  \\
    \midrule
    General random & -7.31\pm1.51&18.51\pm1.93 & -3.89\pm0.56&12.80\pm0.86&\\
    Target random &-5.14\pm1.25&16.57\pm1.98&-2.86(0.72)&12.23(1.33)\\
    Target front & -5.60\pm2.21&16.11\pm2.79&-1.83(0.23)&10.29(0.72)\\
    Target back &-6.17\pm1.11&16.23\pm2.00&-2.86(0.51)&11.09(0.69)\\
    Transpose&-18.86&25.71&-4.80&12.80\\
    \bottomrule
  \end{tabular}
}
\caption{WTQ: System performance w.r.t. numerical reasoning. ST stands for short table, ORI stands for original table. We measure the exact match accuracy.}

[How to select the best table...]

\label{wtq_factoid}
\end{table}

==> latex/7-conclusion.tex <==
\section{Conclusion}
In this paper, we have proposed to evaluate three aspects of robustness of TQA systems: retrieval robustness against table structure changes, attention to relevant cells, and aggregation robustness against \st{numerical} value changes.\annetodo{in case we change any of these names, change here too}
We have presented a novel benchmark for a fine-grained analysis of those aspects.  
The main building blocks of our benchmark are targeted table perturbations methods and high-quality human annotations.
Finally, we evaluate a range of architecturally varied state-of-the-art TQA systems, as well as off-the-shelf LLMs.
\red{Our analysis has revealed their advantages and shortcomings, which pave the way for future research on robustness of table question answering systems.}\annetodo{better: finish with a meaningful sentence: what exactly have we found? I think it might actually make sense to end with a single section "Discussion and Conclusion", merging the two sections. The Conclusion feels a bit "empty" atm}

==> latex/_2-benchmark.tex <==
\section{Our Benchmark: \textsc{FREB-TQA}}
\label{sec:benchmark}
%\MMN{after reading the experiment and result sections: do we have a benchmark or a dataset?}
%\textcolor{red}{I think it is a benchmark; 1) provide both data and framework 2) the robut paper call themself a benchmark even if they only provide data}
% v1
\begin{table}[!t]
\small
\centering
%\resizebox{\columnwidth}{!}{%
  \begin{tabular}{@{}lcccccc@{}}
    \toprule
    \textbf{Aspect}&
      \textbf{\#P} &  \textbf{\#Q} &  \textbf{\#QT}&  \textbf{\#R}&  \textbf{\#C}&  \textbf{\#A}\\
    \midrule
    RR-TSC & 64890 &6489&10.05&12.14&7.18&1.02\\
    Shortcuts &6303&2101&14.75&21.44&5.77&1.05\\
    AR-NVC & 4012&2006&14.62&21.70&5.61&1.05\\
    \midrule
    Total & 75205 &8590&10.28&14.42&6.85&1.03\\
    \bottomrule
  \end{tabular}
%}
\caption{
Benchmark statistics. 
\#P and \#Q show the number of perturbations and questions, respectively.  
QT, R, C, and A represent average  question length in terms of tokens, number table rows, number of table columns and \MM[answer cell]{number of cell composing an answer}, respectively. 
RR-TSC, 
Shortcuts and AR-NVC stand for retrieval robustness against table structure changes, shortcuts usages in retrieval and aggregation robustness against numerical value changes, respectively.
%\MMN{In general, tables do not follow identical style. They must do so. Headers should be bold or not to be. font size should be all small. Do not use resizbox that hurts the style of the tables Check for all tables. }
}
\label{perturbation_statistics}
\end{table}

% original table
% \begin{table}[!t]
% \small
% \centering
% %\resizebox{\columnwidth}{!}{%
%   \begin{tabular}{@{}lccccccc@{}}
%     \toprule
%     \textbf{Type} &\textbf{Aspect}&
%       \textbf{\#P} &  \textbf{\#Q} &  \textbf{\#QT}&  \textbf{\#R}&  \textbf{\#C}&  \textbf{\#A}\\
%     \midrule
%     EQ& RR-TSC& 64890 &6489&10.05&12.14&7.18&1.02\\
%     RQ&Shortcuts&6303&2101&14.75&21.44&5.77&1.05\\
%     RQ&AR-NVC&4012&2006&14.62&21.70&5.61&1.05\\
%     \midrule
%     Total & - & 75205 &8590&10.28&14.42&6.85&1.03\\
     
%     \bottomrule
%   \end{tabular}
% %}
% \caption{
% Benchmark statistics. \textit{EQ} and \textit{RQ} stand for extraction and reasoning questions, respectively. \textit{P}, \textit{Q}, \textit{QT}, \textit{R}, \textit{C}, \textit{A} stand for perturbations, questions, average question tokens, average table rows, average table columns and average answer cell, respectively. \textit{RR-TSC}, \textit{Shortcuts} and \textit{AR-NVC} stand for retrieval robustness against table structure changes, shortcuts usages in retrieval and aggregation robustness against numerical value changes, respectively.
% %\MMN{In general, tables do not follow identical style. They must do so. Headers should be bold or not to be. font size should be all small. Do not use resizebox that hurts the style of the tables Check for all tables. }
% }
% \label{perturbation_statistics}
% \end{table}

FREB-TQA (\textbf{F}ine-grained  \textbf{R}obustness \textbf{E}valuation \textbf{B}enchmark  for \textbf{T}able  \textbf{Q}uestion  \textbf{A}nswering) evaluates the robustness of TQA systems in three aspects: 
%
(1) \firstaspect , 
(2) \secaspect , and
% % retrieval robustness against relevent content changes 
(3) \thirdaspect .
%
\MM[Our benchmark is illustrated in Figure \ref{fig:framework}. ]
{Figure \ref{fig:framework} demonstrates these aspects. }
\MM[Corpus statistics of the benchmark can be found in \tref{perturbation_statistics}. ]{}

To \MM[better study  robustness aspects related to retrieval vs.\ aggregation separately]{disentangle these aspects}, we distinguish between two question types: 
extraction questions (EQs) and reasoning questions (RQs). 
EQs refer to those whose answers can be retrieved from tables while RQs refer to those requiring an  aggregation, i.e., performing numerical operations over several cell values. 
Since the source datasets do not distinguish between these question types, we propose automatic methods to identify each question type. 



For each question type, we define a set of perturbations to address the fine-grained aspects of robustness evaluation,
as shown in Figure \ref{fig:framework}. 

For EQs, we design 
perturbations for evaluating retrieval robustness against table structure changes (RR-TSC). 
These perturbations
alter the table structure but not contents. 
We propose new target-based perturbations %and table transposing 
apart from commonly studied row and column perturbations (Section \ref{sec:tsr}).

For RQs, we design perturbations to study shortcuts usages in retrieval and aggregation robustness against numeric value changes (AR-NVC).
Perturbations for studying shortcut usages center on changes w.r.t. relevant cells. We follow the definition of previous work \cite{Ye2023LargeLM} that relevant cells are the subpart of table (evidence) essential for answering questions. 
An example of relevant cells is shown in the red rectangle in Figure \ref{fig:framework}.
The perturbations include masking out relevant cells, shuffling relevant rows and columns, and escaping the entire table (Section \ref{sec:su}).
As for AR-NVC, we propose two perturbations: cell (numeric)\footnote{We perturb cell values that are numeric. Thus we do not distinguish between cell values and numeric values in AR-NVC.} value changes affect/not affect answers (Section \ref{sec:nrr}).
Our motivation is that a robust system should perform aggregations correctly regardless of numeric value changes.
In other words, systems should adapt answers according to the changes in cell values. 
This is important for TQA systems because it prevent systems from memorizing certain values, thus fail for a different distribution.

%from the values of several table cells.\annetodo{too vague: maybe, the answer is composed by performing numerical operations and aggregation or reasoning over several cells? or just "require the systems to compose the answer from the values of several table cells"?}

\subsection{Source datasets}
\label{sec:source_dataset_section}
We create our benchmark using four frequently used TQA datasets: WikiTableQuestions (WTQ) \citep{Pasupat2015CompositionalSP}, WikiSQL \citep{Zhong2017Seq2SQLGS}, Sequential Question Answering (SQA) \citep{Iyyer2017SearchbasedNS}, and Tabular And Textual dataset for Question Answering (TAT) \cite{Zhu2021TATQAAQ}.
TAT, in particular, features a collection of questions requiring numerical reasoning, which is not reflected in the other three datasets.
We report the statistics of these source datasets in \aref{source_dataset_overview}. 

\subsection{EQs and RQs selection}
\label{sec:qtc}

\begin{table}[t]
\small
\centering
%\footnotesize
  \begin{tabular}{lcc}
    \toprule  
    \textbf{Model}&
     \textbf{EQ}  & \textbf{RQ} \\
      \midrule
    LLaMA2 & 74.27& 57.02
    \\
   % Falcon & 43.1 & 6.3 & 11.0 & 48.7 & 92.2 & 63.7 \\\midrule
   % Dolly & 57.9 & 19.4 & 29.1 & 51.1 & 85.5 & 64.0 \\\midrule    
    Rule-based & 75.23 & \textbf{83.42}\\ 
    Combined & \textbf{93.81}& 60.17 \\
    \bottomrule
  \end{tabular}%
 \caption{Accuracy over models' predictions for 100 EQs (extraction questions) and 100 RQs (reasoning questions) sampled from WTQ. The random baseline is 50.0. Bold values are the best performances.}%\MM[Classification results]{Precision (P), recall (R) and (F) scores of examined question type classifiers} on the 200 instances sampled from the WTQ dev set. The random baseline is 50.0.}
  \label{model_selection}
\end{table}

Since the source datasets vary in annotations, we apply different strategies to obtain EQs and RQs.
For SQA, TAT and WikiSQL, we can leverage existing annotations.
For WTQ, however, no annotations are available and we need to design high-precision selection models. 

\textbf{Selecting EQs and RQs from TAT, SQA and WikiSQL} is based on existing annotations in the source datasets. 
For TAT\footnote{As answers can be in table or in texts, we select questions whose answers are only from tables.}, we select questions requiring no comparison and no mathematical operations as EQs. 
Otherwise, the questions are regarded as RQs.
For SQA, we filter out following-up questions, as we do not target the
conversational question answering setting. We further filter out questions whose answers involve more than one cells to align with the answer distributions of other data sets. 
The remaining questions are all EQs and, thus no RQ is selected from SQA.
For WikiSQL, we select questions whose aggregation label is 0 (no aggregation) as EQ.
We do not select RQ from the dataset as it features mostly EQs.\footnote{We notice in WikiSQL, instances with aggregation label other than 0 do not need aggregation for most of the cases.}

%We first introduce methods and models for the question type classification.
%Then we \MM[illustrate]{introduce their performance as baselines on }\MM[how they are applied on different]{the four source} datasets \MM[for the purpose of selecting]{to separate} extraction and reasoning questions.

\textbf{To select EQs and RQs from WTQ}, we design the following three models and test them on 100 EQs and 100 RQs sampled from WTQ and manually annotated for question types.
%The question type labels are annotated by humans.
Details about the annotation can be found in the \aref{annotations}.
\begin{description}
    \setlength{\itemsep}{0pt}
    \setlength{\parskip}{0pt}
    \setlength{\parsep}{0pt}

\item[Rule-based] 
%\heiketodo{why not say "word-based" or "rule-based"? (It's a bit more specific and, if you want to be very correct, your way of selecting EQs/RQs from TAT, SQA and WikiSQL is also a heuristic)}
We first use string match to detect if answers are in the tables or not. 
If not, we regard the question as RQ. 
If yes, we run POS-tagging on the question to detect whether it contains comparative or superlative words, as they suggest comparing cells, leading to aggregations. 
If the question contains such words, we regard it as RQ. 
Otherwise, we regard it as EQ.
\item[LLM] We prompt an open-source LLM, LLaMA2-13b, to label if a question is EQ or RQ.
The prompt we use is shown in Appendix \ref{llm_prompts}. 

\item[Combined approach] We first use the rule-based approach on a question.
If the question is RQ, we keep the label. 
Otherwise, we run LLaMA2 on the question to obtain the final label.
%\annetodo{consider explaining this top-down earlier, see what works best later}
\end{description}

We select one best model for each question type, based on accuracy over models' predictions.  
This is because we want model-predicted EQs and RQs to be real EQs and RQs as much as possible.
When we use the best model to select EQs and RQs from the whole WTQ, we then have a high quality set of questions. 
The results are shown in \tref{model_selection}. 
Based on the results, we use the combined approach to select EQs and the rule-based approach to select RQs.

We follow \citet{Zhao2023RobuTAS} to remove questions asking about positions (e.g., \textit{What is the name of the actor in the first row?}).
We obtain a set of positional words\footnote{We gather position prepositions (suggesting position) and ordinal numbers (suggesting order) in English to construct the set.} and discard questions containing words in the list.



%We do not focus on building a general model for question type classification, because our main goal is to exhaustively obtain EQs and RQs from the source datasets. 

%As WikiSQL features mostly simple \MMN{vs what? did you define it?} extraction questions, we do not select reasoning questions from it. 

%\MM[]{Thus, we rely on the high-quality of annotations in the WTQ evaluation set and use it to compare the question type classification models (see 
%\MMN{What do we learn from the results above?}

%For processing \MMN{be more specific? What is this processing?} the full datasets for WTQ and WikiSQL, we select the best models based on precision. 
%We use precision because we want the proportion of correct predictions \MMN{did you define correct predictions? task is distinguishing extraction and reasoning} to be as high as possible. 


%For WTQ, We run the combined approach for selecting extraction questions and use the heuristic method for selecting reasoning questions.\annetodo{why this special treatment?}
%For WikiSQL, we select questions that do not need aggregation functions (this is provided in the annotations) as the extraction questions.
%We run the combined approach on the rest of the data to exhaustively select extraction questions. 
%As the data set do not feature reasoning questions, we do not construct the reasoning set based on WikiSQL. \annetodo{?!? I am a bit confused which method was used on which dataset and why} \heiketodo{I agree that this subsection needs to be made clearer; maybe a figure could help; maybe a more result-orientied description could help --- something like ``we use approach X and our analysis on 200 instances confirms that it is better than alternative approaches''; whatever you choose, I think this subsection would benefit a lot from re-structuring and shortening}
%\MMN{while there are some revisions, I think it's not clear yet. You introduced four source datasets. Now for each of them (or groups of them) explain how you split their questions into reasoning and extraction. 
%} 
%\heiketodo{I think the new version of 3.2 is much more focused than earlier versions; I like it's structure and motivation now}

\subsection{Perturbations for evaluating RR-TSC}

\label{sec:tsr}

\citet{Lin2023AnIT} observe that in WikiSQL, answers appear early in the tables, e.g., first row/columns. 
We test if systematic position biases could be observed across source datasets.
To do so, we design target-based row/columns perturbations.
We also introduce table transposing to evaluate systems' robustness against new table strutures. 
%\textcolor{red}{To study the retrieval robustness against table structure changes (RR-TSC), we design perturbations based on three principles:
%1) Focusing on table structures instead of table contents. 
%2) Revealing biases of answer positions in systems if any.
%3) Demonstrating systems' robustness against new table structures.}
%\MMN{consider or introduce or propose? and why ONLY these? }  
\heiketodo{I agree with Mohsen that we need a motivation for each perturbation: why is it necessary / what does it help us to show?}
\begin{description}
    \setlength{\itemsep}{0pt}
    \setlength{\parskip}{0pt}
    \setlength{\parsep}{0pt}
\item[Random row/column shuffling] We randomly shuffle tables row-wise (or column-wise). This perturbation shows models' robustness to table structure changes in retrieval generally.
%\MM[]{:} Randomly \MM[shuffling]{rearranging} the table rows \MM[or columns]{(or columns)}\MM[.]{,}
%\item[Target row/column random]\MM[]{:} We use string match to detect if a row/column contains answers or not (if yes, referred as \MM[ target rows/columns]{a target row/column}). \MMN{Is shuffle a precise verb? How can we shuffle one row/column?} 
%We move the target rows/columns randomly within the table.

\item[Target row front/middle/bottom]
%\MM[]{:} 
We use string match to detect if rows or columns contain answers or not (if yes, referred to as target rows/columns).
We partition tables into three equal-length parts, referred to as the front, middle and bottom parts.
Target rows are moved to each part respectively. 
\textcolor{red}{The partition number three is decided (12/5) based on the averaged row number in the total extraction set (12) and the number of seeds we run for the perturbation (5).
We aim to have target rows moved to every part of tables.
This perturbation can reveal biases of answer positions in systems.} 


%\MMN{How many instances in TAT have 9 rows? This does not conclude to the above experimental setting decision.}
%If more partitions, target rows have less room to be shuffled. 
%If fewer, positional preference of models might not be shown.
%\MMN{motivation needs to be stronger? What does it help us learn? }

\item[Target column front/back] 
%\MM[]{:}
%\MMN{Are front/back precise words? front seems to refer to the face of an object based on Oxford dictionary. }
We partition tables into two parts and referred to them as the front and back parts.
The partitioned is obtained similarly as how we obtained the number for rows.
We move the target columns to the front/back of a table. 

\item[Transpose] To evaluate the robustness against new table structures, 
%\MM[]{:} 
\MM[we transpose the whole table so that columns become rows and rows become columns. ]{we switch the content of a table from columns to rows, or vice versa to create transposed tables.}
\textcolor{red}{\MM[Since headers need to be specified for pre-trained TQA systems, we use indices as the new header after transposing the table.]{
To ensure TQA systems do not use information captures in headers to overcome this perturbation, we transform each header to an index. 
}
\MM[We do that because in reality one might not know the location of header (the first row or column or both).]{} }
\end{description}
%Our perturbations differ from those in prior studies \citep{Yang2022TableFormerRT, Zhao2023RobuTAS} in: 
%1) They are build on instances with EQs.
%2) New target-based perturbations are introduced to study models' preference w.r.t. answer locations.
%3) Table transposing is introduced to test systems' robustness on new table structures. 

%\annetodo{what is target-based shuffling? has not been introduced}
%\MMN{Should you move this part to related work? You should have introduced your perturbations (not in details) in the introduction. So in related work you can talk about your differences. }
%\textcolor{red}{Agree}


%\st{as the new perturbation to test models' robustness on new table structure without changing the information contained.}
%\annetodo{Rewrite this section such that the various methods are explained immediately when they are introduced. You could also first list the perturbations and then add the sentence stating the difference vs prior work.}


%Three different features of our perturbations from previous studies are:\annetodo{In contrast to prior studies (citations), our benchmark creates perturbation data as follows.} 

% AF: typesetting hint to save space (use across paper)
%\begin{description}
%    \setlength{\itemsep}{0pt}
%    \setlength{\parskip}{0pt}
%    \setlength{\parsep}{0pt}
%\item[Title:] text
%\end{description}

%\MMN{I was lost here! What has happened to these perturbations? We just defined them? It's confusing because in question type classifier we report the experimental setting and results. However, for perturbation, we just define them.}
%\textcolor{red}{We just define them.}

\subsection{Perturbations for evaluating shortcuts usages in retrieval}
\label{sec:su}
%\MMN{there is no ''against'' in this perturbation? suggestion: use identical style for naming. }}
As \citet{Gupta2022RightFT} point out, for the table NLI task, systems can derive correct answers without referring to target cells. 
\textcolor{red}{Motivation starts from here:}To test if this is also \MM[true]{valid} in TQA (masking out relevant cells) and what kinds of shortcuts exist (relevant rows/columns perturbations and escaping tables), we introduce the following perturbations:
%\annetodo{moved this up here as it motivates all of these settings}

\begin{description}
    \setlength{\itemsep}{0pt}
    \setlength{\parskip}{0pt}
    \setlength{\parsep}{0pt}

\item[Masking out relevant cells] 
We \MM[evaluate]{investigate} to what extent \MM[]{TQA} systems bypass relevant cells to derive answers by \MM[masking out relevant cells]{masking them out}.
The relevant \MM[cells]{} annotations are \MM[]{borrowed} from \citet{Ye2023LargeLM} for WTQ. 
We test the validity of these annotations first as they are obtained from LLMs. 
Details can be found in Appendix \ref{annotations}.
As for TAT, we use annotations provided in the original dataset to select relevant cells.
\annetodo{The original data? where do the WTQ-provided annotations come in, where your manual annotations? this is unclear}

\item[Relevant rows/columns perturbation] 
\MM[As most TQA models encode positional information of cells apart from cell values, they can leverage it to answer questions.]{This perturbation evaluates to what extent TQA systems use positional information of cells instead of their values.} 
For instance, to answer the question \textit{Who received the least amount of votes?} in Figure \ref{fig:framework}, systems retrieve the last row might be because they learn to relate \textit{least} with the last row during pre-training (as tables are ordered for most of the times).
One distinctive feature between this positional bias and the ones we discuss in Section \ref{sec:tsr} is the former comes from unwanted linkages between questions and cell positions while the latter comes from cell positions purely.
Because of the correlation between cell values and positions, this type of bias is most obvious in questions that need comparing among cells. 
Thus, we study the bias only for questions requiring comparisons.
We select these questions by detecting if they contain superlative or comparative tokens by POS-tagger.  
Then we shuffle the rows or columns containing relevant cells (referred to as relevant rows/columns). 
If no shortcut between questions and cell positions is exploited, predictions should remain the same before and after the perturbation.
%\annetodo{how does this differ from target row/column shuffling?}

\item[Escaping table]
\footnote{We do not include perturbations that passing an empty question because we find nearly all systems fail and there hardly exists shortcuts to analyze.} %\MMN{rephrase it, please.}.} 
To understand to what extent systems exploit shortcuts within questions, we escape table information by passing a dummy table which has a header and one cell, both of value \enquote{None}. 
%We do that because pre-trained TQA systems requires tables as input. 
%\MMN{The perturbations seem to be applicable to a very limited systems and not salable and useful for future. If you want to avoid such a review, do not depend the definition of your perturbation on the systems :) }\textcolor{red}{Name changed to be more general!}
We do not mask out all cell values because table information (e.g., row and column numbers) are still available to models.
\annetodo{would still be available? has anyone else done this? explain what information the model could get from such an empty table? (or just omit this and just say that you pass the dummy table)}
\end{description}
%\MMN{Similar to the previous section, what happends to this perturbations? }

\subsection{Perturbations for evaluating AR-NVC\annetodo{adapt this, I will check the paragraph later--but as for above, check if it is clear who did which annotations, on which dataset, what is used. Work with concrete examples (for both categories), refer to your figure.}}
\label{sec:nrr}
One \MM[interesting]{crucial} aspect of robustness not considered by previous studies is the aggregation robustness against numeric value changes (AR-NVC).
%\MMN{The above explanation is very good. However not in a right place. It should be in introduction. Here you just explain your method as the reader should be convinced in already in the intro.}
\textcolor{red}{Inspired by \cite{Stolfo2022ACF}, we study numeric value changes under two circumstances:}  
%\MMN{In what sense? What would be your novel contribution or main difference here?}
\begin{description}
    \setlength{\itemsep}{0pt}
    \setlength{\parskip}{0pt}
    \setlength{\parsep}{0pt}
\item[\textbf{A}nswer \textbf{C}hange (AC)]
%\MM[]{:} 
Given a part of the table where numerical operations are applied on (referred to as short table), one or two cell values are changed, affecting the final answers. 
\textcolor{red}{We investigate if systems can perform correct aggregations and adapt answers to the numeric value changes.}
%We \MM[test]{investigate} if systems \MM[overfit]{are biased} to certain answer numbers. 
An example is shown in Figure \ref{fig:framework}\MM[, where]{.}
\MM[the]{The} votes for \textit{Olsson} changes from \textit{4} to \textit{361}, resulting the change in answer (from \textit{Olsson} to \textit{Leslie}).
%\MMN{Does the example show the bias? If not, can you show it?}

\item[(Answer) Not Change (NC)]\annetodo{No Answer Change} Given a short table, one or two cell values are changed without affecting the final answers. 
\textcolor{red}{We investigate if systems predict correct answers based on their biases to certain numbers. 
For instance, for the example in Figure \ref{fig:framework}, systems might be capable of comparing \textit{15} and \textit{4}. 
However, if we change the votes for \textit{Leslie} form \textit{15} to \textit{1500}, without changing the answer, systems might face difficulties as \textit{1500} might not fall into the cell values distribution during pre-training. } 
%\MMN{How did you get to AC and NC abbreviations? best scientific writing practice suggest not using non-standard acronyms.  }
\end{description}

\textcolor{red}{While changing numeric values and answers is easy and can be automatically done in \citet{Stolfo2022ACF}, given no irrelevant numbers appear in the question formulation. 
Doing that in the context of table can be no trivial, as tables usually contain irrelevant numbers to answering a question.}
To this end, we create a human-annotated perturbation dataset for TQA, focusing on numeric values changes.
To do so, we ask three annotators to 1) \textbf{identify short tables: the subpart of tables that numerical operations are applied \MM[on]{to}}. 
We do not \MM[simply]{} \MM[give]{provide} annotators \MM[]{with} the relevant cells used in Section \ref{sec:su} because they might not provide sufficient information for answering a question. 
An example is shown in Figure \ref{fig:framework}, where relevant cells are marked by a red rectangle. 
Though the relevant cells are essential for answering the question, passing them alone does not provide models with sufficient information to compose the answer \textit{Olsson}.
2) \textbf{Change one or two cell values in the identified tables either affect or not affect the answer}.
We only change one or two cells to reduce the workload of annotators while still obtaining the perturbations\MM[we want]{}.  
We filter out instances where annotators find unanswerable. 
This results in 1469 questions from WTQ and 537 from TAT in total.
To \MM[test]{assess} the validity of the AC and NC perturbations, we randomly sample 50 AC and 50 NC instances from each reasoning set. 
Then, we ask two annotators who are not involved in the above \MM[perturbations]{perturbation} creation to provide the answers given the changed tables and questions. 
We calculate agreement among the answers provided by the two annotators as well as the answers from the perturbations, mounting up to Fleiss $\kappa$-score of 0.87 for WTQ and 0.61 for TAT, which shows good and moderate agreement \MM[]{,} respectively \cite{McHugh2012InterraterRT}.
%\MMN{citation for the good and moderate please}. 
We examine the cases where annotators do not agree in the 100 examples from TAT (as the score is lower than that of WTQ), and find this is attribute to difference of the positive or negative sign of the values. For instance, for the question \textit{What is the change in total personnel expenses from 2018 to 2019?}
The change can either be positive or negative.

%\MMN{
%Please think about the presentation of this section. It's not yet coherent. It looks like you made many small decisions for specific systems. The output of the section is benchmark. The output is not shown here. What about bring table 1 to the end of this section?
%}

%\MMN{Now that I look at Table 1 in detail. I think we need a "total" row (if not a complete separate table) to show the statistics of our benchmark. The current version of the table is detailed statistics of what portion of our benchmark comes from what source dataset. I think we don't have to split the benchmark with respect to source datasets right?}






==> latex/_5-discussion.tex <==
\section{Discussion}
\paragraph{System robustness} 
GPT-3.5 is more sensitive to table structural changes than other systems.\annetodo{can we rule out that it doesn't simply employ shortcuts / its knowledge in those cases, too?}\annetodo{would you assume that its pretraining data contains less tables than that of OmniTab?} 
It can also exploit more shortcuts without depending on relevant cells or tables than other systems due to its large pre-training corpora. 
We find pipeline approaches where either relevant cells or SQL queries are generated first could help addressing the issue.\annetodo{how did you find this? the Binder system performed worst, or not very well in terms of drops?}
However, one caveat is that using LLMs to parse table and questions into the intermediate representations can still cause unrobustness.
We suggest future studies focus on pipeline approach with open-source LLMs where the robustness of the first stage can be controlled (via fine-tuning, knowledge injection etc). 
OmniTab is generally the most robust systems across all perspectives. 
However, it fails for instances out of its pre-training distribution, e.g., transposed tables. 
Fine-tuning could help but not much.\annetodo{??}
If one's test instances happen to resemble the typical Wikipedia tables, Omnitab should suffice. 
However, Omnitab and pre-trained TQA systems are not good at dealing with unanswerable questions and arithmetic questions (See the TAT results in Appendix \ref{tat_reasoning}). Neither are they robust to numerical value changes. \annetodo{I would really be interested in complete out-of-domain performance, e.g., on scientific tables or other types of tables}

\paragraph{Perturbations}
We discover column perturbations degrade performance as well as robustness more than row perturbations when the structure of table changes. 
This is different from the results in \citet{Zhao2023RobuTAS}. 
We think two reasons attribute to this: 
1) The separation of extraction and reasoning questions help with disclosing the real effect of column shuffling on table structure robustness. 
2) Since most tables in our benchmark features more rows than columns. 
Columns shuffling brings in more change to the table than rows. 

\paragraph{Effects of table length on structure robustness}
We look into the relationship between table size and variation percentage. To do what, we categorize table based on its cell numbers into 6 bins and plot the averaged variation percentage against these bins.\footnote{We select bins are not in equal distance to ensure each bins have similar number of instances.} Results are shown in Figure \ref{length}. We find generally larger tables suffer more in terms of robustness.\annetodo{who suffers?} This shows blindly feeding long tables to systems might not be an optimal choice.

\annetodo{I find it a bit hard to pinpoint the exact new findings here - what exactly are the new things that we learned that we didn't already know, and what are the insights ("what did we learn")? What are the consequences? Can you make a bullet point list? What does it mean to compare row vs. column shuffling? (I think this again hints at the issue that column headers may be more important than row headers, not sure how this relates to Wikipedia tables though, I don't know the dataset well enough)}
        
\pgfplotstableread[row sep=\\,col sep=&]{
    interval & Row & Column & Transpose \\
    <40     &4.67  &7.17  & 46.67  \\
    40-60     &6.35 & 8.46  & 56.25 \\
    60-70    & 6.04 & 10.42 & 57.29 \\
    70-100   & 8.95 &9.52 & 62.38 \\
    100-160   & 7.93  & 11.64 & 59.77 \\
    >160      &11.36 &13.45 & 62.79 \\
    }\mydata
\begin{figure}
\begin{tikzpicture}[font=\small]
    \begin{axis}[
            yline,
            %bar width=.2cm,
            x=1cm,
            enlarge x limits={abs=0.6cm},
            enlarge y limits=false,
            width=0.5\textwidth,
            height=.45\textwidth,
            legend style={at={(0.5,0.5)},
                anchor=north,legend columns=-1},
            symbolic x coords={<40, 40-60, 60-70, 70-100, 100-160, >160},
            xtick=data,
            nodes near coords,
            nodes near coords align={vertical},
            ymin=0,ymax=70,
            ylabel={Variation percentage},
            xlabel={Table size}
        ]
        \addplot table[x=interval,y=Row]{\mydata};
        \addplot table[x=interval,y=Column]{\mydata};
        \addplot table[x=interval,y=Transpose]{\mydata};
        \legend{Row, Column, Transpose}
    \end{axis}
\end{tikzpicture}
\caption{Variation percentage against Table size. Results averaged across models and seeds.}
\label{length}
\end{figure}

What we knew
\begin{enumerate}
    \item TQA systems are not robust
    \item GPT3 exhibits highest robustness in Robut paper.
\end{enumerate}

what is new:
\begin{enumerate}
    \item TQA systems are not robust against the table structural change. Omnitab is the most robust system in this aspect. Contradictory to previous studies, LLMs are less robust than fine-tuned TQA systems. Two reasons why the conclusion differs: 1) on extraction data only 2) perturbation to table structure only. Previous studies also perturb header, table contents, which mostly focus on language robustness. We specifically show robustness related with table structural change and shows LLMs are that robust in this regard as one thinks.
    \item We show TQA systems cannot deal with unanswerable questions and output statistics related with the table in most cases. 
    \item We show approaches generating intermediate representations can help with robusntess (by comparing GPT-3.5 with Binder in terms of variation robustness in all aspects.)
    \item We show TaPas leverage most positional bias 
    \item We show shortening table can help GPT-3.5 and Binder with performance as well as robustness against numeric value changes. 
    \item We show all systems are not robust against numeric value changes, especially when answers also change.
    \item We show shorter table exhibit more robustness against table structural change. [I think it all boils down to LM's ability to deal with long texts.]
\end{enumerate}
\paragraph{Robustness enhancement}


%terminology: LM and LLM:
%https://en.wikipedia.org/wiki/Large_language_model


==> latex/backup.tex <==


%\subsection{Perturbations for \blue{Testing} Aggregation Robustness against Numeric Value Changes} %AF: I have a kind of garden path issue when reading this section title, suggestion:
\subsection{Perturbations for Testing Robustness in Aggregating/\wei[]{Comparing} \wei[Numeric]{} Values} % keep it simple(r) :)
\label{sec:nrr}
TQA systems should compose a correct answer to an RQ by aggregating
or comparing values in a table.
%\wei[]{/comparing} \st{numeric} values in a table. 
% AF: was "aggregating  over": (to) aggregate sth. -- does not need a preposition!!
To evaluate this capability, we \green{manually} modify the values of the cells that should be aggregated to answer questions.


\wei[]{Most values modified are numeric values (approx 50\% for WTQ\footnote{The number is different from the 70\% presented in the previous section because we calculate the percentage among the modified cells by annotators here, rather than among the relevant cells.}and 100\% for TAT).}\annetodo{can you specify this better: of the final perturbed version of the dataset, 50\% of the perturbations in WTQ modify numeric values? Does that mean in 50\% of the cases they modified textual cells? If so we should give an example.} 
We define two types of perturbations.

\noindent\textbf{Modify \st{numeric} values to change answers.}  % 
%We modify cell values to change the answers, accordingly. 
This perturbation allows us to study to what extent TQA systems perform correct aggregations and adapt answers to the \st{numeric} value changes accordingly.  
An example is shown in Figure \ref{fig:framework}. 
The votes for \textit{Olsson} is changed from \textit{4} to \textit{361}, resulting in a change of the answer (from \textit{Olsson} to \textit{Leslie}), who now has most votes (\textit{15}). % AF: extended explanation a bit so it also works without actually going back to Fig. 1
\red{add explanation for the counting example with string changes}

\noindent\textbf{Modify \st{numeric} values without changing answers.} %
%We modify cell values so that the answer does change.
This perturbation aims to study if systems articulate correct answers because of their biases to certain \wei[numbers]{values}. 
For instance, in Figure \ref{fig:framework}, systems might be capable of comparing \textit{15} and \textit{4}. 
However, if we change the votes for \textit{Leslie} from \textit{15} to \textit{1500}, without changing the answer, systems might face difficulties as \textit{1500} might not fall into the cell values distribution during pre-training. 

To create data for both types of perturbations, we ask three human annotators to first identify the table cells that numerical aggregations or comparison operate on.
We refer to the part of the table relevant to answering the question as the \textit{shortened table}.
Then, annotators are asked to change one or two \st{numeric} cell values, once resulting in an answer change and once not resulting in an answer change.
%We only change one or two cells to reduce the workload of annotators while still obtaining interesting perturbations.   
We filter out instances which annotators find unanswerable. 
To assess the quality of the output of these perturbations, for each perturbation type, we randomly sample 50 instances created using this type from each dataset, resulting in 200 instances in total.
Then, we ask two annotators who were not involved in the perturbation creation to provide the answers given the changed tables and questions.
\wei[]{We compute the exact match accuracy of answers provided by the two annotators, which mount up to 92.5\% and 93.5\%. Most of the wrong cases are attributed to the plus/minus sign when the questions ask about change.}\annetodo{are these errors due to the first or due to the second step?}

==> latex/commands.tex <==
% Additional packages
\usepackage{xspace}
\usepackage{graphicx}
\usepackage{enumitem}
\usepackage{xcolor}
\usepackage{tikz-dependency}
\usetikzlibrary{shapes,arrows}
\usepackage{amssymb}
\usepackage{float}
\usepackage{todonotes}

\usepackage{hyperref}       % hyperlinks
\usepackage{url}            % simple URL typesetting
\usepackage{booktabs}       % professional-quality tables
\usepackage{amsfonts}       % blackboard math symbols
\usepackage{nicefrac}       % compact symbols for 1/2, etc.
\usepackage{natbib}
\usepackage{doi}


\usepackage{caption}
\usepackage{subcaption}

\usepackage{lscape}
%\usepackage{soul} % for highlighting text in different colors
\usepackage{longtable} % tables on multiple pages
\usepackage{multirow}
\usepackage{dsfont}

\hyphenation{WikiHow}

\setlist[description]{leftmargin=\parindent,labelindent=0pt}


\newcommand{\blue}[1]{\textcolor{blue}{#1}}
\newcommand{\camerareadyblue}[1]{\textcolor{black}{#1}}

\definecolor{darkgreen}{rgb}{0, 0.75, 0}
\newcommand{\red}[1]{\textcolor{red}{#1}}
\newcommand{\green}[1]{\textcolor{darkgreen}{#1}}
%\newcommand{\green}[1]{#1}
\newcommand{\orange}[1]{\textcolor{black!20!orange}{#1}}


\newcommand{\enquote}[1]{``#1''}

% Shortcuts for cross-references
\newcommand{\sref}[1]{Sec.~\ref{#1}}
\newcommand{\aref}[1]{Appendix~\ref{#1}}
\newcommand{\srefplural}[1]{Sections~\ref{#1}}
\newcommand{\srefshort}[1]{\ref{#1}}
\newcommand{\tref}[1]{Table~\ref{#1}}
\newcommand{\fref}[1]{Figure~\ref{#1}}

\renewcommand{\vec}[1]{\mathbf{#1}}


% Colored todonotes
\definecolor{talita}{rgb}{0.635,0.998,0.722}
\definecolor{anne}{rgb}{0.8,0.8,1}
\definecolor{wei}{rgb}{0.998,0.722,0.635}
\definecolor{heike}{rgb}{0.4, 0.8, 0.4}
\definecolor{final}{rgb}{1, 1, 0.6}

\newcommand{\talitatodo}[2][talita]{\todo[color=#1,size=\footnotesize]{\textbf{#1:} #2}}
\newcommand{\annetodo}[2][anne]{\todo[color=#1,size=\footnotesize]{\textbf{#1:} #2}}
\newcommand{\weitodo}[2][wei]{\todo[color=#1,size=\footnotesize]{\textbf{#1:} #2}}
\newcommand{\heiketodo}[2][heike]{\todo[color=#1,size=\footnotesize]{\textbf{#1:} #2}}
\newcommand{\finaltodo}[2][final]{\todo[color=#1,size=\footnotesize]{\textbf{#1:} #2}}

%\newcommand{\talitatodo}[2][talita]{}
%\newcommand{\annetodo}[2][anne]{}
%\newcommand{\sophietodo}[2][sophie]{}
%\newcommand{\heiketodo}[2][heike]{}
%\newcommand{\finaltodo}[2][final]{}

\newcommand{\anne}[1]{\textcolor{violet}{[AF: #1]}}
\newcommand{\sophie}[1]{\textcolor{orange}{[SH: #1]}}

%Mohsen
\usepackage{color}
\usepackage{soul}


\newcommand{\MM}[2][]{\textcolor{black}{#2}}
%\newcommand{\MMN}[2][]{\textcolor{brown}{\textbf{MM}: #2}}
% \newcommand{\MM}[2][]{\textcolor{black}{#2}}

\newcommand{\wei}[2][]{\textcolor{black}{#2}}

\newcommand{\heike}[2][]{\textcolor{black}{#2}}


% TODO: linguistic examples!
\newcounter{example}
\newenvironment{example}[1][]{\refstepcounter{example}\par
	\textbf{Example~\theexample. #1} \rmfamily}{}

% tables ...
\usepackage{array}
\newcolumntype{L}[1]{>{\raggedright\let\newline\\\arraybackslash\hspace{0pt}}m{#1}}
\newcolumntype{C}[1]{>{\centering\let\newline\\\arraybackslash\hspace{0pt}}m{#1}}
\newcolumntype{R}[1]{>{\raggedleft\let\newline\\\arraybackslash\hspace{0pt}}m{#1}}
\usepackage{rotating}

% highlight in different colors
\newcommand{\hlc}[2][yellow]{ {\sethlcolor{#1} \hl{#2}} }

% mark changes in text for quicker reviewing
\newcommand{\newcontentstart}{\red{new}}
\newcommand{\newcontentend}{\red{endnew}}

\newcommand{\extraHeightOverviewTable}{2pt}


% Paper-specific commands


==> latex/history_paragrph.tex <==

\subsubsection{Questions selection using annotations}
\label{question_classification}\annetodo{the method described in this section is a bit unclear to me}
For SQA, we filter out following-up questions whose positions are not 0, as we do not target the conversational question answering setting. 
We further filter out questions whose answers involve more than one cells to align with the answer distributions of other data sets.
The questions selected are extraction questions and no reasoning questions are obtained for SQA.
With regards to TAT, in terms of extraction questions, we focus on the type of questions whose answers are from tables (since TAT is a hybrid TQA data set), requiring no comparisons and mathematical operations.
In contrast, instances involves comparisons and mathematical operations are categorized as reasoning questions. 
As for WikiSQL, we additionally add questions whose aggregation label is 0 (which means no aggregation) to the extraction data set.
To construct the positional words list. we first gather common positional words in English.
Then we use string match to select the most appeared words in WTQ training set questions. 
The following list contains the positional words we used in this study:
[first, last, top, bottom, before, previous, latter, after, next, below, above]

\begin{figure}[!h]
    \centering
    \includegraphics[width=0.65\columnwidth]{rule_base_flowchart.pdf}

    \caption{Flow chart of rule based and combined selection of extraction and reasoning questions.EQ and RQ stand for extraction and reasoning questions respectively.}
    \label{fig:flowchart}
\end{figure}



\begin{table}
\centering
\resizebox{0.7\columnwidth}{!}{%
  \begin{tabular}{lrrrrrr}
    \toprule  &
      \multicolumn{3}{c}{Extraction} &
      \multicolumn{3}{c}{Reasoning} \\\midrule
     & $P$ & $R$ & $F_{1}$ & $P$ & $R$ & $F_{1}$ \\
      \midrule
    Baseline & .23 & .50& .31 & .77 & .50 & .61 \\\midrule
    Llama2 & .42 & .47 & .44 & .84 & .81 & .82 \\\midrule
    falcon & .26 & .08 & .12 & .77 & .93 & .85 \\\midrule
    dolly & .03 & .19 & .23 & .78 & .87 & .82 \\\midrule    
    heuristic & .45 & .85 & .59 & \textbf{.94} & .69 & .80 \\\midrule    
    combo & \textbf{.85} & .33 & .47 & .83 & .98 & .09  \\
    \bottomrule
  \end{tabular}%
  }
 \caption{Classification results on the 438 instances sampled from the WTQ dev set. The number of extraction and reasoning questions are 100 and 338 respetively.}
  \label{classification_results}
\end{table}



\subsubsection{Shortcuts usages}
\label{shortcut_results}
\begin{table}[!h]
\centering
\resizebox{\columnwidth}{!}{%
  \begin{tabular}{lcccccccc}
    \toprule
      & {ET} & {MRel} & {NoP} & {MRan} & {RelRow} & {VP\_row}&{RelCol}&{VP\_col}  \\
    \midrule
    TAPEX & 8.84 & 9.57 &52.26& $-6.50(\pm9.44)$ & $-1.52(\pm0.35)$ &$9.96(\pm0.44)$ &
    $-5.05(\pm0.50)$&$13.39(\pm0.44)$  \\
    OmniTab & 7.76 & 12.55 & \textbf{58.12} & $-2.26(\pm0.27)$ & $-0.69(\pm0.39)$&$6.68(\pm0.22)$&-2.62(\pm0.15)$& $8.03(\pm0.21)$\\
    TaPas & \textbf{2.80} & \textbf{8.21}&  47.02  &$-2.62(\pm0.37)$ & $-0.90(\pm0.42)$ &$7.44(\pm0.12)$ &$-2.85(\pm0.31)$&$7.04(\pm0.45)$ \\
    GPT-3.5 & 6.95 & 16.52 & 42.06& $-2.94(\pm0.41)$ & $-1.97(\pm0.43)$ &$16.01(\pm0.51)$ &$-3.95(\pm0.44)$& $17.78(\pm0.98)$ \\
    LLAMA2 & 7.44 & 11.91&  35.92 & $-0.13(\pm0.29)$ &$-2.40(\pm1.73)$  &$17.96(\pm3.58)$& $-2.65(\pm1.56)$&$19.30(\pm2.93)$ \\
    Binder &6.86&11.62& 45.67   &$-2.60(\pm0.23)$ & $-1.53(\pm0.55)$ &$8.75(\pm0.45)$& $0.02(\pm 0.51)$ & $12.94(\pm0.44)$ \\
    \bottomrule
  \end{tabular}
}
\caption{WTQ: system performance w.r.t. shortcut usages. ET stands for escape table, MRel stands for mask relevant cells, MRan stands for mask random cell, RelRow stands for relevant row shuffling and RelCol stands for relevant col shuffling. For MWT and MRel, we report the exact match scores, for the rest, we report exact match difference. For all values, the smaller (absolute value), the better. We did not report results for TaPas and Llama2 as this data set is too challenging for these systems.}
\label{tat_shortcut}
\end{table}


\begin{table}[!h]
\centering
\resizebox{\columnwidth}{!}{%
  \begin{tabular}{lcccccccc}
    \toprule
      & {ET} & {MRel} & {NoP} & {MRan} & {RelRow} & {VP\_row}&{RelCol}&{VP\_col}  \\
    \midrule
    TAPEX & 3.53 & 5.38 &9.65& $-0.56(\pm1.44)$ & $-1.54(\pm0.48)$ &$4.96(\pm0.44)$ &
    $-2.93(\pm0.34)$&$5.45(\pm1.02)$  \\
    OmniTab &3.90 & 6.12 & 10.02 & $-0.56(\pm1.58)$ & $-1.04(\pm0.59)$&$1.60(\pm1.82)$&-2.71(\pm0.69)$& $4.49(\pm1.13)$\\
    %TaPas & \textbf{2.80} & \textbf{8.21}&  47.02  &$-2.62(\pm0.37)$ & $-0.90(\pm0.42)$ &$7.44(\pm0.12)$ &$-2.85(\pm0.31)$&$7.04(\pm0.45)$ \\
    GPT-3.5 & 0 & 1.73 & 36.17& $-2.48(\pm1.65)$ & $-2.97(\pm0.68)$ &$11.33(\pm1.61)$ &$-6.37(\pm0.79)$& $16.69(\pm1.98)$ \\
    %LLAMA2 & 1.44 & 11.91&  35.92 & $-0.13(\pm0.29)$ &$-2.40(\pm1.73)$  &$17.96(\pm3.58)$& $-2.65(\pm1.56)$&$19.30(\pm2.93)$ \\
    Binder &0&1.01& \textbf{37.65}   &$-1.53(\pm0.97)$ & $-1.42(\pm0.65)$ &$4.35(\pm1.94)$& $-2.56(\pm 0.69)$ & $7.63(\pm1.24)$ \\
    \bottomrule
  \end{tabular}
}
\caption{TAT: system performance w.r.t. shortcut usages. ET stands for escape table, MRel stands for mask relevant cells, MRan stands for mask random cell, RelRow stands for relevant row shuffling and RelCol stands for relevant col shuffling. For MWT and MRel, we report the exact match scores, for the rest, we report exact match difference. For all values, the smaller (absolute value), the better }
\label{wtq_shortcut}
\end{table}

%Another question is whether systems are taking random guess when predicting on the BC questions given no table information, or there exists some preferences over one of the choices? If systems are taking random guess, the number of BC instances that are correctly and incorrectly predicted should be somewhat similar. Therefore, the odds of correct predictions against incorrect predictions should be 100\%. We calculate the odds for each system and find that systems are not taking random guess. More specifically, for TAPEX, OmniTab and GPT-3.5, the odds are around 35\%, whereas for Llama2 and Binder, the odds are around 5\%. The number suggests systems generally predict more incorrectly than correctly (which is the preferred behaviour given no table information is provided) and systems are not randomly guessing the answers. 

%by looking at the percentage of incorrectly predicted instances whose answers are also 1. As the numbers are all much higher (range between 30-100\%) than 0, this means systems do not only give answer 1 due to overfitting. Interestingly,


%\begin{table}[!h]
%\centering
%\resizebox{1\columnwidth}{!}{%
%  \begin{tabular}{lcccccc}
%    \toprule
%      & {Odds (BC-c)} & {Pct (BC)} & {Pct (Pred1-inc)}& {Pct (Pred1)} & {Pct-other}\\
%    \midrule
%    TAPEX &36.00  & 55.10 & 33.33 & 30.61& 14.29\\
%    OmniTab &33.33 & 59.30 &60.00 &20.93&19.77 \\
%    TaPas & 0  & 0 &37.78 &90.32&9.68  \\
%    GPT-3.5 &36.91  & 71.43 & 52.59 &0&28.57  \\
%    LLAMA2 & 5.15 &62.50& 91.11 &  25&12.5 \\
%    Binder & 6.25 & 66.67 &1.0 & 0 &33.33 \\
%    \bottomrule
%  \end{tabular}
%}
%\caption{WTQ: Escape table statistics. Might need to move it to appendix.}

%\label{escape_table}
%\end{table}


%\begin{table}[!h]
%\centering
%\resizebox{1\columnwidth}{!}{%
%  \begin{tabular}{lccccccc}
%    \toprule
%      & {Odds (BC-c)} & {Pct (BC)} & {Pct (Row-inc)}& {Pct (Row)} & {Pct-other} & {Unexplainable}\\
%    \midrule
%    TAPEX &31.62  & 46.23 & 18.18 & 8.49& 45.28&30.19\\
%    OmniTab &26.71 & 30.94 &15.22 &28.06&41.01&29.50 \\
%    TaPas & 0.99  & 2.20 &1.79 &61.44&37.36&26.37  \\
%    GPT-3.5 &30.77  & 26.23 & 3.33 &15.85&57.92&44.81 \\
%    LLAMA2 & 29.94 &35.61& 67.74 &  7.58&56.82&43.18 \\
%    Binder &17.24 & 39.47 & 35.14 & 31.58 &  28.95& 17.11\\
%    \bottomrule
%  \end{tabular}
%}
%\caption{WTQ: Mask relevant cells statistics. Might need to move it to the appendix.}

%\label{mask_relevant_cells}
%\end{table}

\subsection{Numerical reasoning robustness: TAT}
\label{tat_reasoning}
\begin{table}[!h]
\centering
\resizebox{1\columnwidth}{!}{%
  \begin{tabular}{lcccccc}
    \toprule
      & {ST} & {AC} & {NC} & {ORI} & {AC-VP} & {NC-VP} \\
    \midrule
    TAPEX &10.17  & 2.79 & 6.70 &9.68 &8.38&2.23\\
    OmniTab &12.96 & 1.68 &6.33&10.06 &6.33&2.05 \\
    %TaPas & 48.57  & 48.50 &48.84 &41.09&16.39&3.81  \\
    GPT-3.5 &\textbf{46.37}  & \textbf{38.92} & 45.93& 36.30 &26.82& 14.71 \\
    %LLAMA2 & 13.88 & 11.77& 12.79 &  32.59&32.45&6.31 \\
    Binder & 41.19 &36.94 &42.26 &\textbf{37.78} &9.50&8.19  \\
    \bottomrule
  \end{tabular}
}
\caption{TAT: System performance w.r.t. numerical reasoning. ST stands for short table, ORI stands for original table. We measure the exact match accuracy and variation percentage (compared with the short table setting).}

\label{numerical_reasoning}
\end{table}



\begin{table}[t]
\small
\centering
%\footnotesize
  \begin{tabular}{lcccccc}
    \toprule  &
      \multicolumn{3}{c}{Extraction} &
      \multicolumn{3}{c}{Reasoning} \\\midrule
     & $P$ & $R$ & $F_{1}$ & $P$ & $R$ & $F_{1}$ \\
      \midrule
    LLaMA2 & 74.3 & 46.2 & 57.0 & 60.7 & 84.4 & 70.6 \\\midrule
   % Falcon & 43.1 & 6.3 & 11.0 & 48.7 & 92.2 & 63.7 \\\midrule
   % Dolly & 57.9 & 19.4 & 29.1 & 51.1 & 85.5 & 64.0 \\\midrule    
    Heuristic & 75.2 & 84.6 & 79.6 & \textbf{83.4} & 72.1 & 77.3 \\\midrule    
    Combined & \textbf{93.8} & 34.4 & 50.4 & 60.2 & 98.1 & 74.6  \\
    \bottomrule
  \end{tabular}%
 \caption{\MM[Classification results]{Precision (P), recall (R) and (F) scores of examined question type classifiers} on the 200 instances sampled from the WTQ dev set. The random baseline is 50.0.}
  \label{classification_results_balanced}
\end{table}


%For WikiSQL and WTQ, either no annotations can be used to classify question types or the annotations do not suffice\footnote{We also use part of the annotations to add up the extraction questions for WikiSQL, see \aref{question_classification}}
%\MMN{how do you define if they suffice or not?}. 
%We select the best automatic method \MMN{automatic?} from LLMs, heuristics and combined approaches based on \MM[a manual]{an} evaluation step \MMN{step or set?}. 
%We manually annotate 200 instances (100 extraction and 100 reasoning questions) from the development set of WTQ.\MM[\footnote{To get 100 extraction and 100 reasoning questions, we end up annotating 428 questions in total as the type distribution is
%not balanced. We show the model results in the appendix. The best model remains unchanged.}]
{
%To acquire 100 extraction and 100 reasoning questions, we end up annotating 428 questions in total as the type distribution is not balanced. 
}




\subsubsection{Escape table}\annetodo{In this discussion, it is somewhat unclear where the results come from: is this a manual analysis? based on which results? first, also state what the performance drop is for escaping the table. Reviewers can completely ignore the appendix! they could just write here, not understandable, not backed up by the study/results, and reject your paper!}
We identify three types of instances that models are still capable of predicting correctly when escaping the table and plot the distributions of these types.\annetodo{I do not fully get what the ground total is here: all questions of these types, or are you showing the distribution within the errors that the systems make? But you said for these questions, the systems actually still predict the correct answer?} The results are shown in Figure \ref{escape_distribution}. 

\begin{itemize}
    \item BC (binary choice): Answers are directly shown in questions. For instances: \textit{Did belfast royal academy have more or less total finals than ballyclare high school?}
    \item Pred1: models return answers with 1.
    \item Others: any cases other than the above two. %either the questions can be answered with world knowledge or there might be data leakage that enables systems predict correct answers without table information.
\end{itemize}


Most systems feature large distributions of BC errors except from TaPas. 
This might be because, as the only classification model, TaPas needs to select relevant cells first and then performs aggregations. 
Given no table is provided, it is impossible for it to select correct cells. 
As a result, it predicts incorrectly for all BC questions. 

With regards to predicting answer 1, the distribution is very different among systems. 
Binder and GPT-3.5 do not predict any answers 1, whereas the percentage of answer 1 is the highest for TaPas. 
We rule out the possibility that systems overfit fine-tuning data, thus predicting with 1. 
The analysis can be found in Appendix \ref{shortcut_results}. 
Majority of questions leading to this behaviour contain "how many". 
We believe systems return the number of row/column/cell, which is 1 when using the proxy table. 
The phenomenon can also be observed in TAT.
End-to-end systems are not pre-traiend with unanswerable question-table pairs, thus they cannot output "unanswerable". 
Interestingly, they output table row/column/cell related statistics when being asked "how many", even though the tables are not related with the questions.

Lastly, in terms of the Others case, GPT-3.5 and Binder noticeably have a large proportion of this type.
When looking into the questions, we find most of them can be solved by common knowledge. 



\pgfplotsset{testbar/.style={
    ybar stacked,
    width=.5\textwidth,
    height=0.1\textwidth,
    legend style={at={(0.73,0.24)},
                anchor=north,legend columns=-1},
    ymajorgrids = true,
    ymin=0,ymax=100,
    xtick = data, xticklabels = {TAPEX, OmniTab, TaPas, GPT-3.5, Llama2, Binder},
    yticklabels={,,,},
    label style={font=\small},
    legend style={font=\small},
    tick align = outside, ytick pos = left,
    bar width=3mm, y=0.3mm,
    nodes near coords style={font=\tiny},
    nodes near coords={\pgfmathprintnumber{\pgfplotspointmeta}\%}, % <-- prints % sign after y coordinate value
    yticklabel={\pgfmathprintnumber{\tick}\%},% <-- prints % sign after x tick value
    nodes near coords align={center}, % <-- horizontal alignment centered of nodes 
    enlarge x limits=0.1, % <-- Adds vertical space so to not crop the bars
}}
\begin{figure}
    \centering
\begin{tikzpicture}[font=\small]
    \begin{axis}[testbar]
        \addplot coordinates{(0,55.10) (1,59.30) (2,0) (3,71.43) (4,62.50) (5,66.67) };
        \addplot coordinates{(0,30.61) (1,20.93) (2,90.32) (3,0) (4,25) (5,0)};
        \addplot coordinates{(0,14.29) (1,19.77) (2,9.68) (3,28.57) (4,12.5) (5,33.33)};
        \legend{BC, Pred1, Others}
    \end{axis}
\end{tikzpicture}
 \caption{Distribution of three types of errors for different systems.}
    \label{escape_distribution}
\end{figure}



%OmniTab:
%number of mc question: 51, 0.5930232558139535
%number of p1 question: 14,0.16279069767441862
%number of mc corrct predict: 153
%total mc instances:204, correct mc percent (should not be): 0.25, incorrect mc percent (shoule be):0.75
%number of p1 corrct predict: 13
%total mc instances:27, correct mc percent (should not be): 0.5185185185185185, incorrect mc percent (should be):0.48148148148148145
%================================

%TAPEX:
%number of mc question: 54, 0.5510204081632653
%number of mc corrct predict: 150
%total mc instances:204, correct mc percent (should not be): 0.2647058823529412, incorrect mc percent (shoule be):0.7352941176470589
%===============================

%TaPas:
%number of mc question: 0, 0.0
%number of mc corrct predict: 204
%total mc instances:204, correct mc percent (should not be): 0.0, incorrect mc percent (shoule be):1.0
%==============================

%GPT-3.5:
%number of mc question: 55, 0.7142857142857143
%number of mc corrct predict: 149
%total mc instances:204, correct mc percent (should not be): 0.2696078431372549, incorrect mc percent (shoule be):0.7303921568627451
%=============================

%llama:
%number of mc question: 10, 0.625
%number of mc corrct predict: 194
%total mc instances:204, correct mc percent (should not be): 0.049019607843137254, incorrect mc percent (shoule be):0.9509803921568627

\subsubsection{Mask relevant cells} 
When masking relevant cells which provide key information for answering a question, systems should fail to answer the questions. 
We look into the error types and find systems fail on BC questions, questions asking total row numbers. 
The rest \st{part}\annetodo{how many are these?} might be due to data leakage: systems have already seen the tables or questions during pre-training. 
We plot the percentage of this type for all systems and the results are shown in Figure \ref{mask_relevant}.



\pgfplotsset{testbar/.style={
    ybar,
    width=.5\textwidth,
    height=0.1\textwidth,
    legend style={at={(0.73,0.24)},
                anchor=north,legend columns=-1},
    ymajorgrids = true,
    ymin=0,ymax=50,
    xtick = data, xticklabels = {TAPEX, OmniTab, TaPas, GPT-3.5, Llama2, Binder},
    yticklabels={,,,},
    label style={font=\small},
    legend style={font=\small},
    tick align = outside, ytick pos = left,
    bar width=3mm, y=0.3mm,
    nodes near coords style={font=\tiny},
    nodes near coords={\pgfmathprintnumber{\pgfplotspointmeta}\%}, % <-- prints % sign after y coordinate value
    yticklabel={\pgfmathprintnumber{\tick}\%},% <-- prints % sign after x tick value
    nodes near coords align={center}, % <-- horizontal alignment centered of nodes 
    enlarge x limits=0.1, % <-- Adds vertical space so to not crop the bars
}}
\begin{figure}
    \centering
\begin{tikzpicture}[font=\small]
    \begin{axis}[testbar]
        \addplot coordinates{(0,30.19) (1,29.50) (2,26.37) (3,44.81) (4,43.18) (5,17.11) };
        %\legend{Others}
    \end{axis}
\end{tikzpicture}
 \caption{Distribution of the rest type for different systems.\annetodo{I do not get this statistic, see my comment above}}
    \label{mask_relevant}
\end{figure}

We find GPT-3.5 and Llama2 have the highest percentage of the type that might due to data leakage.
This is no surprise as LLMs are pre-trained on much larger amount of data than TQA systems.
As for Binder, the number is low.
Binder queries LLMs by transforming questions and tables into SQL queries.
LLMs might not have seen these intermediate task data.  
%As for end-to-end systems, TaPas features a smaller percentage of questions cannot be answerable than TAPEX and OmniTab.
%carry out an error analysis on instances that systems can still predict. 
%in this setting. Similar as in the escape table setting, systems take advantage of binary classification questions. Another type of instances that systems are still capable of correctly predicting is the question asking row numbers (indirectly). For this type of questions, though table contents are masked, still systems can infer row numbers by table structures. We focus on analyzing the rest case in a qualitative manner. 

%We eliminate the cases where key information is still available to models due to wrong masking annotations and cases where masking key information does not change the original answers (e.g., the second largest is of the same values as the largest when asking what is the largest values), the rest cases should fail the systems as they are unanswerable.

%[Can it be the case the systems can guess the masked rows are the key information thus return correct answers when asking how many? Maybe run further experiment on this]

%We attribute this to either data leakage or system is capable of guessing the key information is replaces by ''. For instance, for the question: how many times did brazil play west germany during the 1982 season? with original answer 1, the key row brazil play against west germany is masked with '', systems might guess the empty row is the key row, thus return 1. We validate this by created new tables (so systems cannot have seen it during pre-training or fine-tuning) with how many questions and mask important row with ''. We find systems fail for most of the cases [This is just an assumption, need to run experiment to validate!]. This means systems are not inferring the answers based on masked row numbers, thus leaving the possibility of data leakage during pre-training. We manually go through each systems and report the percentage of this type (among all correctly predicted). We think LLMs might already seen the table data during its pre-training, thus resulting correct predictions even masking key information. Why systems can still correctly answer these questions given key info is masked? 


\subsubsection{Positional bias}
For reasoning questions, systems might exploit cells' positions to infer answers from, as tables in pre-training data might be ordered based on cell values. 
To look into how much positional bias systems exploit, we conduct our analysis on reasoning questions requiring comparisons (e.g., \textit{Which nation earned the most gold medals?}). 
Instances requiring numerical reasoning typically fall into three categories w.r.t. aggregations in our data sets: comparing, counting and arithmetic. 
We choose\annetodo{what do you mean by "we choose"?} comparing because positional bias is the easiest to exploit in this case.

We look into the percentage of instances requiring comparing in two cases: 
1) where predictions change after shuffling relevant rows or columns (either correct to incorrect or incorrect to correct) 
2) where predictions do not change and remain correct before and after shuffling. 
Our intuition is that if systems do not exploit shortcuts, there should not be any preference over predictions between the two cases. 
The results are shown in Figure \ref{relevant_shuffle_percent}.

We find that for TaPas, the percentage of comparing questions\annetodo{why did the percentage of question types change? I can't quite follow the reasoning here, why we can deduce from this that the model uses positional bias, or whether sth else is going on. What exactly would the positional bias be? Rows that are compared are adjecent, or sth. else?} is much bigger in \textsc{Preds\_change} than in \textsc{Preds\_correct}. 
This suggests TaPas leverages positional shortcuts most compared with other systems. 
Additionally, the percentage of comparing questions in \textsc{Preds\_correct} is higher than that in \textsc{Preds\_change} for LLMs.
The trend is the opposite for end-to-end pre-trained TQA systems. 
This might indicate generally LLMs exploits less positional shortcuts than pre-traiend TQA systems. 

\pgfplotstableread[row sep=\\,col sep=&]{
    interval & pred_change & change_error & pred_correct & correct_error \\
    TAPEX     &54.25 &2.36 & 50.49&0.56   \\
    OmniTab     &54.10 &1.98  & 53.18&0.16 \\
    TaPas    & 72.36 & 2.65 & 47.30&0.33 \\
    GPT-3.5   & 47.79 &1.02 & 53.39&0.62 \\
    Llama2   & 53.80  & 5.41 & 55.79&1.06\\
    Binder  &47.89  &1.36 & 53.05 & 0.27    \\
    }\mydata
\begin{figure}
\begin{tikzpicture}[font=\small]
    \begin{axis}[
            ybadifferent r,
            bar width=.2cm,
            x=1cm,
            enlarge x limits={abs=0.6cm},
            enlarge y limits=false,
            width=0.5\textwidth,
            height=.45\textwidth,
            legend style={at={(0.50,1.00)},
                anchor=north,legend columns=-1},
            symbolic x coords={TAPEX, OmniTab, TaPas, GPT-3.5, Llama2, Binder},
            xtick=data,
            xticklabel style={anchor= east,rotate=45 },
            nodes near coords,
            every node near coord/.append style={yshift=5pt,anchor=south,{font=\tiny}},
            nodes near coords align={vertical},
            ymin=40,ymax=80,
            ylabel={Percentage},
            xlabel={}
        ]
        \addplot 
        plot [error bars/.cd, y dir=both, y explicit]
        table[x=interval,y=pred_change,y error plus=change_error, y error minus=change_error]{\mydata};
        \addplot 
        plot [error bars/.cd, y dir=both, y explicit]
        table[x=interval,y=pred_correct,y error plus=correct_error, y error minus=correct_error]{\mydata};
        \legend{\textsc{Preds\_change}, \textsc{Preds\_correct}}
    \end{axis}
\end{tikzpicture}
\caption{Percentage of instances whose questions require comparing. \textsc{Pred\_change} is the prediction change setting and \textsc{pred\_all} is the prediction unchanged (correct) setting. The percentage of comparing questions of the total reasoning data set is 48.08\%.}
\label{relevant_shuffle_percent}
\end{figure}


%co-co
%inco-co+co-inco
%tapex 
%[0.5368217054263565, 0.5348837209302325, 0.5475728155339806, 0.5484496124031008, 0.5447470817120622]
%0.5424949872011465 0.005593412766862379
%=======================================
%tapex
%[0.5339805825242718, 0.5092592592592593, 0.49572649572649574, 0.4636363636363636, 0.5175438596491229]
%0.5040293121591026 0.023696417400493778

%omnitab
%[0.5298013245033113, 0.5342237061769616, 0.533003300330033, 0.5307820299500832, 0.5313531353135313]
%0.531832699254784 0.0015841459479344821
%omnitab
%[0.5555555555555556, 0.5333333333333333, 0.5070422535211268, 0.5641025641025641, 0.5405405405405406]
%0.5401148494106242 0.01976761308054505

%tapas
%[0.47468354430379744, 0.474468085106383, 0.47478991596638653, 0.46638655462184875, 0.47489539748953974]
%0.4730446994975911 0.0033320742985977086
%tapas
%[0.7108433734939759, 0.6785714285714286, 0.7469879518072289, 0.75, 0.7317073170731707]
%0.7236220141891607 0.02645746103257725

%chatgpt
%[0.5349462365591398, 0.5300546448087432, 0.5290858725761773, 0.5454545454545454, 0.5297297297297298]
%0.5338542058256671 0.0061635278792855205
%chatgpt
%[0.47904191616766467, 0.480225988700565, 0.4945652173913043, 0.4722222222222222, 0.46368715083798884]
%0.47794849906394904 0.010185029677604785

%llama2
%[0.5691823899371069, 0.5538461538461539, 0.5709876543209876, 0.5433962264150943, 0.5521235521235521]
%0.557907195328579 0.010571085340355646
%llama2
%[0.47058823529411764, 0.5800865800865801, 0.47297297297297297, 0.5807860262008734, 0.5854700854700855]
%0.5379807800049259 0.054089170253715416

%binder
%[0.4819004524886878, 0.47692307692307695, 0.4777777777777778, 0.4822222222222222, 0.47544642857142855]
%0.47885399159663866 0.002724850636096074
%binder
%[0.5192307692307693, 0.5434782608695652, 0.5425531914893617, 0.5098039215686274, 0.5376344086021505]
%0.5305401103520948 0.013564141305266047



%\paragraph{Take away messages} When encountered with unanswerable questions, pre-trained TQA systems,  especially TaPas, tend to give table related statistics (e.g., row/column/cell numbers) rather than outputting \textit{unanswerable}. 
%LLMs, due to their large pre-training corpora, can still solve questions even when relevant cells are removed.\annetodo{this statement is quite broad!!}
%In terms of positional bias, we find TaPas leverage it the most than other systems.  



\begin{table}[!h]
\centering
\resizebox{1\columnwidth}{!}{%
  \begin{tabular}{lcccccc}
    \toprule
      & {ST} & {AC} & {NC} & {ORI} & {AC-VP} & {NC-VP} \\
    \midrule
    TAPEX &48.03  & 46.05 & 47.23 & 47.55&30.00&5.65\\
    OmniTab &\textbf{54.69} & \textbf{52.18} &\textbf{54.42} &\textbf{52.79}&26.46&4.76 \\
    TaPas & 48.57  & 48.50 &48.84 &41.09&16.39&\textbf{3.81}  \\
    GPT-3.5 &51.70  & 50.27 & 52.59 &38.91&23.20& 8.78 \\
    LLaMA2 & 13.88 & 11.77& 12.79 &  32.59&32.45&6.31 \\
    Binder & 50.88 & 49.94  &50.00 &42.99 &\textbf{14.56}&7.96  \\
    \bottomrule
  \end{tabular}
}
\caption{WTQ: System performance w.r.t. numerical reasoning. ST stands for short table, ORI stands for original table. We measure the exact match accuracy and variation percentage (compared with the short table setting).}

\label{numerical_reasoning_wtq}
\end{table}

\begin{table}[!h]
\centering
\resizebox{1\columnwidth}{!}{%
  \begin{tabular}{lcccccc}
    \toprule
      & {ST} & {AC} & {NC} & {ORI} & {AC-VP} & {NC-VP} \\
    \midrule
    TAPEX &10.17  & 2.79 & 6.70 &9.68 &8.38&2.23\\
    OmniTab &12.96 & 1.68 &6.33&10.06 &6.33&2.05 \\
    %TaPas & 48.57  & 48.50 &48.84 &41.09&16.39&3.81  \\
    GPT-3.5 &\textbf{46.37}  & \textbf{38.92} & 45.93& 36.30 &26.82& 14.71 \\
    %LLAMA2 & 13.88 & 11.77& 12.79 &  32.59&32.45&6.31 \\
    Binder & 41.19 &36.94 &42.26 &\textbf{37.78} &9.50&8.19  \\
    \bottomrule
  \end{tabular}
}
\caption{TAT: System performance w.r.t. numerical reasoning. ST stands for short table, ORI stands for original table. We measure the exact match accuracy and variation percentage (compared with the short table setting).}
\end{table}

\paragraph{Take away messages} Shortening table helps with numerical reasoning. The effect is more obvious for LLMs than TQA systems.\annetodo{Above you mentioned LLMs as one type of TQA systems (though I don't quite agree with this way of phrasing it).}
Pipeline approaches suffer less than end-to-end systems when cell values and answers change.


As our perturbations involve positional change of target cells, systems might retrieve wrong cells not because of unrobustness to table structural change but because the target cells flow over models' maximum input window. 


\begin{table*}[t]
\small
\centering
\resizebox{\textwidth}{!}{%
  \begin{tabular}{lccccccc}
    \toprule
    \multirow{2}*{\textbf{Question type}} &\textbf{Data set}&
      \textbf{\#Perturbations} &  \textbf{\#Question} &  \textbf{\#Question tokens}&  \textbf{\#Row}&  \textbf{\#Column}&  \textbf{\#Answer cell}\\
    \midrule
    & & 77211 &8590&10.28&14.42&6.85&1.03\\
    \midrule
     \multirow{4}*{\textbf{Extraction}} & WTQ \citep{Pasupat2015CompositionalSP} & 2050 & 205 & 9.51& 17.26 & 6.23 & 1.05 \\
     & WikiSQL\cite{Zhong2017Seq2SQLGS} & 60130 & 6013 & 10.10 & 11.93 & 7.31 & 1.02 \\
    & SQA\cite{Iyyer2017SearchbasedNS} & 1570 &157 &8.63 & 15.60 &5.94 & 1.0  \\
    & TAT\cite{Zhu2021TATQAAQ} & 1140 & 114 &10.40 &9.46 & 3.77 &1.0  \\
    \midrule
    \multirow{2}*{\textbf{Reasoning}} & WTQ & 9093 & 1562 & 10.05 & 25.76 & 6.40 & 1.07  \\
     & TAT & 3228 & 539 & 13.63 & 8.91 & 3.93 & 1.01 \\
     
    \bottomrule
  \end{tabular}
}
\caption{
Benchmark statistics. \textcolor{red}{Extraction questions are questions that can be answered by retrieving relevant cells while reasoning questions require additional aggregations.}
}
\label{perturbation_statistics}
\end{table*}

\pgfplotstableread[row sep=\\,col sep=&]{
    model & compare & compare_error & non_compare & non_compare_error \\
    TAPEX     &10.24 &0.52 & 9.70&0.73   \\
    OmniTab     &7.37 &0.47  & 6.02&0.19 \\
    TaPas    & 10.98 & 0.29 & 4.04&0.44 \\
    GPT-3.5   & 16.62 &0.66 & 16.40&0.56 \\
    Llama2   & 17.11  & 2.76 & 12.89&1.50\\
    Binder  &9.47  &0.28 & 9.07 & 0.64    \\
    }\mydata
\begin{figure}
\begin{tikzpicture}[font=\small]
    \begin{axis}[
            ybar,
            bar width=.2cm,
            x=1cm,
            enlarge x limits={abs=0.6cm},
            enlarge y limits=false,
            width=0.5\textwidth,
            height=.45\textwidth,
            legend style={at={(0.5,1.00)},
                anchor=north,legend columns=-1},
            symbolic x coords={TAPEX, OmniTab, TaPas, GPT-3.5, Llama2, Binder},
            xtick=data,
            xticklabel style={anchor= east,rotate=45 },
            nodes near coords,
            every node near coord/.append style={yshift=5pt,anchor=south,{font=\tiny}},
            nodes near coords align={vertical},
            ymin=3,ymax=23,
            ylabel={Variation percentage},
            xlabel={}
        ]
        \addplot 
        plot [error bars/.cd, y dir=both, y explicit]
        table[x=model,y=compare,y error plus=compare_error, y error minus=compare_error]{\mydata};
        \addplot 
        plot [error bars/.cd, y dir=both, y explicit]
        table[x=model,y=non_compare,y error plus=non_compare_error, y error minus=non_compare_error]{\mydata};
        \legend{\textsc{Compare}, \textsc{No\_compare}}
    \end{axis}
\end{tikzpicture}
\caption{}
\label{}
\end{figure}

==> latex/introduction_original.tex <==
Table provides an efficient way to store and present information. \annetodo{Tables are a structured format that provide an efficient way ...} 
As a result, it is\annetodo{they are} widely used in various domains \cite{Zhu2021TATQAAQ,Chen2020HybridQAAD,Desai2021TabLeXAB}. 
Since tables can be lengthy and feature different types of data\annetodo{such as text or numbers}, e.g., texts, numbers, how to accurately and effectively query information from tables with natural language has been an important and long-studied topic \citep{Zelle1996LearningTP,Pasupat2015CompositionalSP,Dong2016LanguageTL,Lin2023AnIT}.\annetodo{This sentence is hard to parse. Also, it is unclear whey the querying in NLP research follows from the length and various data types. I would disentangle these aspects.} 

The task is known as \textbf{Table Question Answering} (TQA).\annetodo{this sentence connects so strongly to its preceding sentence that I'd not use a paragraph break in between.}
It aims to provide answers w.r.t. questions and tables through table understanding
and reasoning \cite{jin2022survey}.\annetodo{In this paper, we address the task of TQA, which aims to provide answers ... --> the survey says "table encoding and reasoning" -- I do not like the term "understanding" here, let's try to avoid it as much as possible. None of the models we have looked at can claim to "understand" tables.}
Considering\annetodo{Consider} the examples in Figure \ref{example}:
to answer the question \textit{Who received the least amount of votes?}, one has to understand different types of data, for instance, natural language. In addition to that, understanding table structure to locate relevant cells (columns \textit{Candidate} and \textit{Votes}) is also essential.\annetodo{I still see the shared titles example - has this been updated?}
Last but not least, sometimes, reasoning is required to derive the final answer (\textit{least}--> the smallest number).

Though many systems\annetodo{Here, I would probably add a high-level description of these systems: TQA systems have addressed these challenges using X (.....) and Y (....) --> give the reader already some qualitative information, what type of solutions exist} \cite{Herzig2020TaPasWS,Liu2021TAPEXTP,Jiang2022OmniTabPW,Cheng2022BindingLM,Ni2023LEVERLT,Lei2023S3HQAAT} have been proposed to address the challenges provided by various TQA data sets \cite{Pasupat2015CompositionalSP,Iyyer2017SearchbasedNS, Chen2020HybridQAAD, Zhu2021TATQAAQ}.
They are shown to be unrobust to perturbations to tables and questions \cite{Yang2022TableFormerRT,Zhao2023RobuTAS}.\annetodo{Here, you might expand a bit: what did the previous studies on robustness find? most important 2-3 points (this leads to the "Gap")} 

However, as stated before, TQA is a comprehensive task requiring different abilities from models (natural language and table structure understanding, numerical reasoning etc).
Previous studies about the robustness of TQA systems do not distinguish these abilities, thus fail to provide insights about in which aspects models are not robust. 
\st{We acknowledge it is important to know generally whether a system is robust or not. 
However, it is more interesting and insightful to look at the different profiles of robustness as the task itself is comprehensive in nature.}\annetodo{remove, not adding much, also you haven't stated it above (in detail)} 

Guided by this idea, for the first time, we propose a general framework for evaluating the robustness of TQA systems in three aspects: table structure robustness, shortcut usages and numerical reasoning robustness.\annetodo{this is too broad! you will not be able to make conclusions here either. Focus on the steps that you really target: identifying the relevant cell(s) (which requires correct identification of row and target), numerical reasoning -- do we also have "combining" several such steps? That could maybe count as some "reasoning"}\annetodo{ I would phrase it like this: which different abilities does it require from humans? -- then say that the previous studies did not take these into account}
The framework can be applied on different types of models (pipeline, end-to-end etc.) and new TQA data sets can be integrated easily.\annetodo{it does not make sense to phrase this wrt the models: the method creates data, it does not do sth with the models}
To the best of our knowledge,  the last two aspects are completely unstudied in previous studies. 
As for the table structure robustness, either previous studies do not look into table structures purely \cite{Zhao2023RobuTAS} because they do not distinguish the different abilities required w.r.t.a question or their perturbation data are synthesized \cite{Sui2023GPT4TableCL}, thus cannot reveal the robustness of systems in real world data.\annetodo{\annetodo{ I would phrase it like this: which different abilities does it require from humans? -- then say that the previous studies did not take these into account}} 

Our contributions are:\annetodo{make the annotation etc. their own contribution. explaining the aspects should go above, the contribution is providing data for it, (maybe proposing to analyse robustness according to these dimensions: but this goes into contribution (1)), performing the analysis.}
\begin{itemize}
        \item We propose a new robustness evaluation framework for TQA, targeting different aspects: table structure robustness, shortcut usages\annetodo{not explained!} and numerical reasoning robustness.
        \item Based on the framework, new perturbation data are provided. Compared with previous studies, our data sets features: 1) distinction between extraction and reasoning questions. 2) numerical reasoning perturbations 3) target-based perturbations for table structure robustness. 
        \item We provide comprehensive analysis for different types of models used in TQA, i.e., end-to-end pre-trained TQA systems, LLMs, approaches combining LLMs with symbolic language. 
    \end{itemize}

Our main findings are: 
1) in terms of table structure robustness, end-to-end models outperform LLMs and LLMs based approaches. However, LLMs can better adapt to new table structure than fine-tuned end-to-end systems. 
2) In terms of shortcut usages, LLMs leverage less positional shortcuts than end-to-end systems and we observe TaPas has the highest tendencies to use positional shortcuts than other models.
3) In terms of numerical reasoning robustness, direct answer generation with generative models faces more difficulties than approaches transforming tables and answers into intermediate stages, e.g., SQL queries then generate answers in a deterministic way when cell values and answers change. 



%apply sometimes apply numerical reasoning \citep{Zhu2021TATQAAQ} or commonsense reasoning \citep{gupta2023temptabqa} over the target cells, as is shown in Figure 1. 


\begin{figure}[!t]
    \centering
    \includegraphics[width=1\columnwidth]{example.pdf}

    \caption{Example of table question answering. The upper table is the original table and lower one is the transposed one. The example is from \cite{Pasupat2015CompositionalSP} and due to length restriction, we only show part of the table. Two types of questions are shown at the right-hand side: extraction questions can be answered by simply extracting cells as answers and reasoning questions require aggregation functions over the relevant cells. }
    %The input sentence (in yellow boxes) is appended with a prompt template (in blue boxes). This prompt is fed into a PBM, and the last hidden representation (in orange boxes) for the \textsc{[MASK]} token is used to predict the label. Attribution scores are extracted based on the predicted label, converted by the verbalizer, e.g., positive --> great, negative --> terrible.}
    \label{example}
\end{figure}

%One of the distinctive features of table data is its semi-structure. 
%It leads to the fact that information stored within the table remains the same regardless of table structural change (e.g., transposing), as shown in Figure \ref{example}. 
%Though efforts have been made to enhance the performance of models for many data sets in TQA \cite{Herzig2020tWS,Liu2021TAPEXTP,Jiang2022OmniTabPW}. 
%They are shown to be unrobust to various perturbations to tables and questions \cite{Yang2022TableFormerRT,Zhao2023RobuTAS}. 
%However, as stated before, TQA is a complicated task requiring different abilities from models.

%\input{latex/main} 

As TQA is a complicated task requiring systems to understand natural language, table structure, and sometimes to reason over selected cells (e.g., summing specific cells), a prediction change caused by an input change, e.g., row orders might be attribute to many reasons. 
Their framework cannot give insights on which aspect systems might not be robust in. In this study, we propose a new robustness evaluation framework that disentangle the robustness of TQA systems into three aspects.   

==> latex/sometable.tex <==

\definecolor{babyblue}{RGB}{204,229,255}

\begin{table*}[t]
\centering
\resizebox{\textwidth}{!}{%
  \begin{tabular}{lcccccccccccc}
    \toprule
    \multirow{2}*{\textbf{Ps}} &
      \multicolumn{6}{c}{\textbf{Exact match difference}} &
      \multicolumn{6}{c}{\textbf{Variation percentage}}  &\\
      \cmidrule(lr){1-7}
      \cmidrule(lr){8-13}
      & {TAPEX} & {OmniTab} & {TaPas} & {GPT-3.5} & {LLaMA2} & {Binder}& {TAPEX} & {OmniTab} & {TaPas} & {GPT-3.5} & {LLaMA2} & {Binder} \\
      \cmidrule(lr){1-7}
      \cmidrule(lr){8-13}
    NP & 84 & \cellcolor{babyblue} 84.57 & 69.71 & 77.71 & 63.43 & 72.57 & 0 & 0 & 0 & 0 & 0 & 0 \\
    \midrule
    R-GR & $-3.09\pm0.46$ & $-1.03\pm0.98$ & $-0.91\pm1.06$ & \cellcolor{babyblue} -0.57\pm1.20 & $-3.43\pm2.20$ & $-2.86\pm1.30$ &  $7.43\pm1.14$  & \cellcolor{babyblue} 4.46\pm0.98 & $7.54\pm1.11$ & $11.31\pm1.42$ & $16.46\pm2.03$ &  $9.03\pm1.51$ \\
    R-TR & $-1.71\pm1.30$ & \cellcolor{babyblue} 0.46\pm0.43 & $-1.14\pm1.70$ & $-0.91\pm1.18$ &$-0.69\pm1.82$  &$-3.66\pm1.33$ & \cellcolor{babyblue} 4.00\pm0.96 & $4.11\pm0.43$  & $6.17\pm1.17$ & $10.06\pm1.79$ & $12.34\pm1.56$ & $10.74\pm2.62$ \\
    R-TF & $-2.17\pm1.17$ & \cellcolor{babyblue} 0.00\pm0.36 &$ 0.57\pm0.89$ & $-0.69\pm1.71$ & $1.26\pm1.27$& $-3.89\pm1.75 & $3.31\pm0.23$ & \cellcolor{babyblue} 2.51\pm0.58 & $4.46\pm0.23$ & $12.80\pm1.83$ &$10.40\pm0.91$  & $11.43\pm2.96$ \\
    R-TM & $-1.03\pm0.56$ & \cellcolor{babyblue} 0.00\pm0.81 & $-1.71\pm0.36$ & $-1.49\pm0.78$ & $-2.40\pm0.56$ & $-3.54\pm2.21$ & \cellcolor{babyblue} 1.71\pm0.00 & $3.43\pm0.36$ & $3.54\pm1.11$ & $11.09\pm1.78$ & $9.71\pm0.72$ & $10.86\pm2.91$\\
    R-TB & $-2.63\pm0.69$ & $-1.03\pm0.84$ & $-0.69\pm0.43$ & \cellcolor{babyblue} -0.46\pm1.37 & $-2.97\pm1.75$ & $-3.43\pm1.20$ & $4.23\pm1.43$ & \cellcolor{babyblue} 3.09\pm0.28$ & $4.57\pm0.36$ & $10.51\pm0.86$ & $14.40\pm0.43$ & $10.06\pm2.19$\\
          \midrule
    C-GR & $-4.91\pm0.93$& \cellcolor{babyblue} -0.91\pm1.28 & $-2.51\pm1.18$ & $-7.31\pm1.51$ & $-6.74\pm2.92$ & $-4.11\pm1.75$ & $11.09\pm2.30$ & \cellcolor{babyblue} 5.94\pm0.78 & $6.17\pm0.84$ & $18.51\pm1.93$& $11.09\pm2.30$ &$10.97\pm1.42$ \\
    C-TR & $-5.26\pm0.98$ & \cellcolor{babyblue} -0.11\pm1.67 & $-1.94\pm1.00$ & $-5.14\pm1.25$ & $-2.17\pm2.94$ & $-3.43\pm1.14$ & $7.77\pm2.57$& \cellcolor{babyblue} 5.60\pm1.32 & \cellcolor{babyblue} 5.60\pm1.27 & $16.57\pm1.98$ & $13.83\pm2.24$ & $10.29\pm2.04$\\
    C-TF & $-3.77\pm0.46$ & \cellcolor{babyblue} -1.03\pm0.56 & $-1.37\pm0.28$ & $-5.60\pm2.21$ & $-5.46\pm3.85$  & $-2.86\pm1.20$  & $6.51\pm1.00$ & \cellcolor{babyblue} 3.77\pm1.12 & $4.34\pm0.28$ & $16.11\pm2.79$ & $15.77\pm2.57$ & $10.86\pm2.48$ \\
    C-TB & $-6.97\pm2.71$ & \cellcolor{babyblue} -1.26\pm0.56 & $-2.40\pm0.91$ & $-6.17\pm1.11$ & $-4.80\pm1.47$ & $-2.97\pm2.41$ & $9.49\pm2.44$ & $5.83\pm0.56$ & \cellcolor{babyblue} 4.46\pm1.37 & $16.23\pm2.00$ & $12.91\pm2.00$ & $10.97\pm1.93$ \\ 
      \midrule
     Tr & -65.14 & -64.57 & -54.86 & \cellcolor{babyblue} -18.86 & -34.29 & -70.86  & 68.57 & 70.29 & 61.71 & \cellcolor{babyblue} 25.71 & 42.29 & 70.86\\
     \midrule
     Tr FT &-43.11 &-41.71 & -46.83& & & & \\
    \bottomrule
  \end{tabular}
}
\caption{WTQ: system performance on extraction data set. \textit{Ps} stands for perturbations. \textit{NP} stands for no perturbation. \textit{R}, \textit{C} and \textit{Tr} stand for row, column and transpose perturbations. \textit{GR},\textit{TR},\textit{TF},\textit{TM} and \textit{TB} stand for general random, target random, target front, target middle, target bottom/back respectively. \textit{FT} stands for fine-tuned. We shade the best performances (minial absolute values) with blue.}
\label{wtq_factoid}
\end{table*}

